METEOR:A Dense, Heterogeneous, and Unstructured Traffic Dataset With Rare Behaviors

We present a new traffic dataset, METEOR, which captures traffic patterns and multi-agent driving behaviors in unstructured scenarios. METEOR consists of more than 1000 one-minute videos, over 2 million annotated frames with bounding boxes and GPS trajectories for 16 unique agent categories, and more than 13 million bounding boxes for traffic agents. METEOR is a dataset for rare and interesting, multi-agent driving behaviors that are grouped into traffic violations, atypical interactions, and diverse scenarios. Every video in METEOR is tagged using a diverse range of factors corresponding to weather, time of the day, road conditions, and traffic density. We use METEOR to benchmark perception methods for object detection and multi-agent behavior prediction. Our key finding is that state-of-the-art models for object detection and behavior prediction, which otherwise succeed on existing datasets such as Waymo, fail on the METEOR dataset. METEOR marks the first step towards the development of more sophisticated perception models for dense, heterogeneous, and unstructured scenarios.

==> figs/Density_Area.tex <==
\begin{figure*}[t]
\centering
   \begin{subfigure}[h]{0.245\textwidth}
    \includegraphics[width=\textwidth]{figs/density/high_d.png}
    \caption{High density.}
    \label{fig: nogameplan}
  \end{subfigure}
  %
 \begin{subfigure}[h]{0.245\textwidth}
    \includegraphics[width=\textwidth]{figs/weather/rain.png}
    \caption{Rainy weather.}
    \label{fig: gameplan}
  \end{subfigure}
 %
   \begin{subfigure}[h]{0.245\textwidth}
    \includegraphics[width=\textwidth, height=2.32cm]{figs/time/night2.jpg}
    \caption{Night time.}
    \label{fig: nogameplan}
  \end{subfigure}
  %
 \begin{subfigure}[h]{0.245\textwidth}
    \includegraphics[width=\textwidth]{figs/urban_rural/rural.png}
    \caption{Rural areas.}
    \label{fig: gameplan}
  \end{subfigure}
 
\caption{\rain~has diverse traffic environments including high density traffic, rainy weather, night-time driving, and rural areas with unmarked lanes.}
  \label{fig: density_area}
  \vspace{-10pt}
\end{figure*}



==> tables/BP.tex <==
\begin{table}[t]%[tbhp]
\centering
\caption{\textbf{Behavior detection results:} We use a video activity prediction model~\cite{bp-model} to perform behavior prediction on our dataset and compare the mAP with a behavior prediction on the HDD.}
% \resizebox{\columnwidth}{!}{
\begin{tabular}{cc}
\toprule
Dataset & mAP \\
\midrule
Honda Driving Dataset~\cite{hdd} & $51.10$ \\
% \midrule
\textbf{\rain} & $\bm{70.74}$ \\
\bottomrule
\end{tabular}
% }
\label{tab: behavior_prediction}
\vspace{-10pt}
% \addtabletext{nomenclature for the TSs refers to the numbered species in the table.}
\end{table}


==> tables/metadata.tex <==
\begin{table}[t]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{ccccccc}
    \toprule[1.25pt]
    \multicolumn{2}{c}{\textit{Area ($\%$)}} & \multicolumn{3}{c}{\textit{Density ($\%$)}} & \multicolumn{2}{c}{\textit{Heterogeneity ($\%$)}}  \\
    \midrule
     Urban & Rural & Low & Medium & High & Het. & Hom.  \\
     
     $76.80$ & $23.20$ & $51.76$ & $29.73$ & $18.49$ & $84.22$ & $15.78$   \\
     
     \midrule
      \multicolumn{2}{c}{\textit{Road type ($\%$)}} & \multicolumn{2}{c}{\textit{Time ($\%$)}} & \multicolumn{2}{c}{\textit{Weather ($\%$)}}& \textit{\# videos}\\
      \midrule
      Smooth & Rough & Day & Night & Normal & Rainy & \multirow{2}{*}{$1250$}\\
      $71.00$ & $29.00$ & $74.25$ & $25.75$ & $90.38$ & $9.62$&\\
     \bottomrule[1.25pt]
    \end{tabular}}
    \caption{\textbf{Dataset statistics:} We report percentage of videos according to various aspects.}
    \label{tab: meta_data}
    \vspace{-10pt}
\end{table}
